Towards Learning-Augmented Peer-to-Peer Networks: Self-Stabilizing Graph Linearization with Untrusted Advice

Distributed peer-to-peer systems are widely popular due to their decentralized nature, which ensures that no peer is critical for the functionality of the system. However, fully decentralized solutions are usually much harder to design, and tend to have a much higher overhead compared to centralized approaches, where the peers are connected to a powerful server. On the other hand, centralized approaches have a single point of failure. Thus, is there some way to combine their advantages without inheriting their disadvantages? To that end, we consider a supervised peer-to-peer approach where the peers can ask a potentially unreliable supervisor for advice. This is in line with the increasingly popular algorithmic paradigm called algorithms with predictions or learning-augmented algorithms, but we are the first to consider it in the context of peer-to-peer networks. Specifically, we design self-stabilizing algorithms for the fundamental problem of distributed graph linearization, where peers are supposed to recover the "sorted line" network from any initial network after a transient fault. With the help of the supervisor, peers can recover the sorted line network in $O(\log n)$ time, if the advice is correct; otherwise, the algorithm retains its original recovery time (i.e., without any supervisor). A crucial challenge that we overcome is to correctly compose multiple self-stabilizing algorithms, that is, one that processes and exploits the advice, and another that does not rely on the advice at all. Our key technical contributions combine ideas from the fields of overlay networks and proof-labeling schemes. Finally, we give a matching lower bound of $\Omega(\log n)$ for the recovery time of any algorithm if the advice can be corrupted, where $n$ is the network size.

==> main-files/Conclusion.tex <==
\section{Conclusion and Future Work} \label{sec:concl}
In this paper, we design and analyse distributed self-stabilizing overlay algorithms, augmented with advice, for converging to a sorted-path topology. Our design of advice has several desirable properties, including being compact and Sybil resistant. Importantly, our algorithms are robust against bad advice, in that they resort to the convergence guarantees with no advice. To the best of our knowledge, we are the first to give such beyond worst-case guarantees, in the framework of algorithms with predictions \cite{MitzenmacherV20,MitzenmacherV22}, for peer-to-peer networks.

Our approach can be generalized to other locally-checkable topologies. Informally, a topology is termed \emph{locally-checkable}, given that every node can observe the states of its neighboring nodes including its own state, if it has the following properties: (1) if the network does not form the topology, at least one node detects a fault; whereas (2) if the network forms the topology, then no node detects a fault; see, e.g., \cite{BernsGP13} for more details. In this work, we exploited the locally-checkable properties of the sorted-path topology to achieve robustness; see, Algorithm \ref{alg:conf-init}. However, researchers have proposed self-stabilizing algorithms for many other locally-checkable topologies \cite{feldmann2020survey}.

To that end, one can generalize our approach, by using the Tree-to-Path algorithm to construct a hypercube on the fly, and then the nodes could rely on the virtual ids suggested by the supervisor to form the target topology. For ensuring that the advice is robust, a (rooted) spanning tree in the target topology (chosen by the supervisor) can be verified by the nodes using the certification of spanning tree \cite{Feuilloley-DMTCS21}. (In our case, the target topology was itself a tree.) Note that this verification (quickly) ensures that the connections suggested by the supervisor form a single connected component. Thus, combining the local checks for the target topology, and the certification of some spanning tree in that topology, one can design robust self-stabilizing algorithms for other topologies.

%For any such topology, we briefly discuss the additional variables required for the flyover algorithms. In particular, a node $u$ can have two variables, namely $u.\mathit{deg}$ and $u.\textit{targ-top}$, where $u.\mathit{deg}$ stores the degree of node $u$ and $u.\textit{targ-top}$ stores the neighboring ids, in the target topology (resp.). Additionally, $u.\textit{tt-vID}$ can store the virtual ids (in the hypercube) of the neighboring nodes in the target topology.

%Using our approach of building a hypercube and routing over it, other important topologies such as Skip graph, De Bruijn graph, etc, can also be formed in (optimal) logarithmic number of rounds. This is an important and relevant problem that has direct applications to distributed hash tables (e.g., \cite{MankuPODC03}), blockchains \cite{DotanACMsurvey21} and distributed machine learning (e.g., \cite{NegliaINFOCOM19}).

We conclude with a few open questions and directions for future work.
\begin{enumerate}
    \item One natural direction is to design an advice that exhibits a smooth correlation between how good the advice is and how much of the target topology is formed. We remark that a key requirement would be a feasible notion of \emph{error} for the advice. For example, if a part of the topology is already formed, the supervisor may not need to provide advice to all the nodes, thereby significantly reducing the message complexity.
    \item Recently, Naor, Parter and Yogev \cite{NaorSODA20} showed that a spanning tree can be verified with only $O(1)$-sized proofs (certificates) and 3-rounds of interaction (between the prover and the network). From the perspective of the supervisor, it is interesting to know if the advice message to each node can be of size at most \emph{sublogarithmic} number of bits.
    \item Further, in practice, it is worth investigating if the supervisor (for e.g., ``prediction serving systems'' \cite{azure, gooogle-cloud, aws, CrankshawNSDI17, olsten-arxiv} in the form of cloud service) can \emph{learn} the reliable links of the network (after repeated failures over time). This information can then be used by the supervisor to work with a (learned) connected subgraph (of the current snapshot) for computing the advice, avoiding nodes to explicitly send their neighborhood for the advice.
\end{enumerate}


